The orbital PDF: general inference of the gravitational potential from steady-state tracers

We develop two general methods to infer the gravitational potential of a system using steady-state tracers, i.e., tracers with a time-independent phase-space distribution. Combined with the phase-space continuity equation, the time independence implies a universal Orbital Probability Density Function (oPDF) $\mathrm{d} P(\lambda|{\rm orbit})\propto \mathrm{d} t$, where $\lambda$ is the coordinate of the particle along the orbit. The oPDF is equivalent to Jeans theorem, and is the key physical ingredient behind most dynamical modelling of steady-state tracers. In the case of a spherical potential, we develop a likelihood estimator that fits analytical potentials to the system, and a non-parametric method ("phase-mark") that reconstructs the potential profile, both assuming only the oPDF. The methods involve no extra assumptions about the tracer distribution function and can be applied to tracers with any arbitrary distribution of orbits, with possible extension to non-spherical potentials. The methods are tested on Monte Carlo samples of steady-state tracers in dark matter haloes to show that they are unbiased as well as efficient. A fully documented \textsc{C/Python} code implementing our method is freely available at a GitHub repository linked from \url{http://icc.dur.ac.uk/data/#oPDF}.

==> makefile <==
MAIN=fit1v1b
OLD=old/fit2v0c
BIB=fitting.bib
STYLE=mn2e_new.bst mn2e-bst.sty mn2e.cls aas_macros.sty 
#lineno.sty

paper:
	latex $(MAIN)
	bibtex $(MAIN)
	latex $(MAIN)
	latex $(MAIN)
	dvipdf $(MAIN)

diff:
	latexdiff $(OLD).tex $(MAIN).tex >diff.tex
	latex diff
	bibtex diff
	@make paper -e MAIN=diff
	@make clean -e MAIN=diff
	
tar: paper
	mkdir tmp
	mkdir tmp/figures
	cp $(MAIN).pdf $(MAIN).tex $(MAIN).bbl $(BIB) $(STYLE) makefile tmp/
	cp figures/*.eps tmp/figures/
	cd tmp;	tar -czhf $(MAIN).tar.gz *; mv $(MAIN).tar.gz ../
	
clean:
	\rm -rf tmp
	\rm -f $(MAIN).aux $(MAIN).log $(MAIN).toc $(MAIN).blg $(MAIN).dvi $(MAIN).ps $(MAIN).out $(MAIN).bbl
ultclean:
	\rm -rf tmp
	\rm -f *.aux *.log *.toc *.blg *.dvi *.ps *.out *.bbl *.backup  *.pdf *.tar.gz

